Markov switching models: an application to roadway safety

In this research, two-state Markov switching models are proposed to study accident frequencies and severities. These models assume that there are two unobserved states of roadway safety, and that roadway entities (e.g., roadway segments) can switch between these states over time. The states are distinct, in the sense that in the different states accident frequencies or severities are generated by separate processes (e.g., Poisson, negative binomial, multinomial logit). Bayesian inference methods and Markov Chain Monte Carlo (MCMC) simulations are used for estimation of Markov switching models. To demonstrate the applicability of the approach, we conduct the following three studies. In the first study, two-state Markov switching count data models are considered as an alternative to zero-inflated models for annual accident frequencies, in order to account for preponderance of zeros typically observed in accident frequency data. In the second study, two-state Markov switching Poisson model and two-state Markov switching negative binomial model are estimated using weekly accident frequencies on selected Indiana interstate highway segments over a five-year time period. In the third study, two-state Markov switching multinomial logit models are estimated for severity outcomes of accidents occurring on Indiana roads over a four-year time period. One of the most important results found in each of the three studies, is that in each case the estimated Markov switching models are strongly favored by roadway safety data and result in a superior statistical fit, as compared to the corresponding standard (non-switching) models.

==> frequency_expl_week_table.tex <==

\tabcolsep=0.5em
\begin{tabular}{|l|l|}
\hline
\bf Variable & \hspace{4cm}{\bf Description}\\
\hline
$\langle\lambda_{t,n}\rangle_X$ & mean accident rate
($\lambda_{t,n}$ for NB), averaged over all values of explanatory
variables ${\bf X}_{t,n}$\\
\hline
$\langle{\rm std}_{t,n}\rangle_X$ & standard deviation of accident
rate ($\sqrt{\lambda_{t,n}(1+\alpha\lambda_{t,n})}$ for NB),
averaged over ${\bf X}_{t,n}$\\
\hline
$p_{0\rightarrow1}$ & Markov transition probability of jump from
state 0 to state 1 as time $t$ increases to $t+1$\\
\hline
$p_{1\rightarrow0}$ & Markov transition probability of jump from
state 1 to state 0 as time $t$ increases to $t+1$\\
\hline
${\bar p}_0$ and ${\bar p}_1$ & unconditional probabilities of
states 0 and 1\\
\hline
$\#$ free par. & total number of free model coefficients
($\beta$-s and $\alpha$-s)\\
\hline
averaged $LL\!$ & posterior average of the log-likelihood (LL)\\
\hline
$\max(LL)$ & for MLE it is the maximal value of $LL$ at convergence;
for Bayesian-MCMC estimation \\
& it is the maximal observed value of LL during the MCMC simulations\\
\hline
marginal $LL\!$ & logarithm of marginal likelihood of data,
$\ln[f({\bf Y}|{\cal M})]$, given model ${\cal M}$\\
\hline
max(PSRF) & maximum of the potential scale reduction factors (PSRF)
calculated separately for all \\
& continuous model parameters, PSRF is close to 1 for converged
MCMC chains\\
\hline
MPSRF & multivariate PSRF calculated jointly for all parameters,
close to 1 for converged MCMC\\
\hline
accept. rate & average rate of acceptance of candidate values
during Metropolis-Hasting MCMC draws\\
\hline
\hline
alpha & the over-dispersion parameter in the negative binomial models\\
\hline
bridm & "number of bridges per mile" quantitative variable
(takes on continuous values)\\
\hline
dep & "median configuration is depressed" indicator variable (dummy)\\
\hline
I70164 & "accident occurring on interstates I-70 or I-164"
indicator variable\\
\hline
intercept & "constant term (intercept)" quantitative variable \\
\hline
ISs & "width of the interior shoulder is less that 5 feet"
indicator variable\\
\hline
maxEA & "maximum of external angles of horizontal curves"
quantitative variable\\
\hline
maxHC & "maximum of reciprocal values of horizontal curve radii"
quantitative variable\\
\hline
maxViK & "maximum of reciprocal values of vertical curve radii"
quantitative variable\\
\hline
OBna & "outside barrier absence" indicator variable \\
\hline
OSs & "width of the outside shoulder is less that 12 feet"
indicator variable\\
\hline
Ramps & "total number of ramps on the viewing \& opposite sides
of the roadway" quant.~variable\\
\hline
Rstrml & "number of ramps on the viewing side per lane per
mile" quantitative variable\\
\hline
spr & "spring season" indicator variable\\
\hline
sum & "summer season" indicator variable \\
\hline
VCnumm & "number of vertical curves per mile"
quantitative variable \\
\hline
wint & "winter season" indicator variable \\
\hline
$X_4$ & "pavement quality index (PQI) average" quantitative
variable \\
\hline
$X_5$ and ln$X_5$ & "road section length" quantitative variable
and its logarithm \\
\hline
$X_{20}$ & "median barrier presence" indicator variable \\
\hline
$X_{23}$ & "interior shoulder presence" indicator variable \\
\hline
$X_{26}$ & "interior rumble strips presence" indicator variable \\
\hline
$X_{32}$ and ln$X_{32}$ & "Average Annual Daily Traffic
(annual average)" quantitative variable and its logarithm \\
\hline
$X_{34}$ & "posted speed limit" quantitative variable \\
\hline
$X_{64}$ & "percentage of single unit trucks (daily average)"
quantitative variable \\
\hline
\end{tabular}



==> frequency_expl_year_table.tex <==

\tabcolsep=0.5em
\begin{tabular}{|l|l|}
\hline
\bf Variable & \hspace{4.0cm}{\bf Description}\\
\hline
$\langle\lambda_{t,n}\rangle_X$ & mean accident rate
($\lambda_{t,n}$ for NB), averaged over all values of explanatory
variables ${\bf X}_{t,n}$\\
\hline
$\langle{\rm std}_{t,n}\rangle_X$ & standard deviation of accident
rate ($\sqrt{\lambda_{t,n}(1+\alpha\lambda_{t,n})}$ for NB),
averaged over ${\bf X}_{t,n}$\\
\hline
$\#$ free par. & total number of free model coefficients
($\beta$-s and $\alpha$-s)\\
\hline
averaged $LL\!$ & posterior average of the log-likelihood (LL)\\
\hline
$\max(LL)$ & for MLE it is the maximal value of $LL$ at convergence;
for Bayesian-MCMC estimation \\
& it is the maximal observed value of LL during the MCMC simulations\\
\hline
marginal $LL\!$ & logarithm of marginal likelihood of data,
$\ln[f({\bf Y}|{\cal M})]$, given model ${\cal M}$\\
\hline
max(PSRF) & maximum of the potential scale reduction factors (PSRF)
calculated separately for all \\
& continuous model parameters, PSRF is close to 1 for converged
MCMC chains\\
\hline
MPSRF & multivariate PSRF calculated jointly for all parameters,
close to 1 for converged MCMC\\
\hline
accept. rate & average rate of acceptance of candidate values
during Metropolis-Hasting MCMC draws\\
\hline
\hline
alpha & the over-dispersion parameter in the negative binomial models\\
\hline
bridm & "number of bridges per mile" quantitative variable
(takes on continuous values)\\
\hline
dep & "median configuration is depressed" indicator variable (dummy)\\
\hline
I70164 & "accident occurring on interstates I-70 or I-164"
indicator variable\\
\hline
intercept & "constant term (intercept)" quantitative variable \\
\hline
ISs & "width of the interior shoulder is less that 5 feet"
indicator variable\\
\hline
maxA & "maximum absolute value of change in grade of a vertical curve"
quantitative variable\\
\hline
maxHC & "maximum of reciprocal values of horizontal curve radii"
quantitative variable\\
\hline
OBna & "outside barrier absence" indicator variable \\
\hline
Rstr & "number of ramps on the viewing side" quantitative variable\\
\hline
Rstrml & "number of ramps on the viewing side per lane per
mile" quantitative variable\\
\hline
tau & \\
\hline
$X_4$ & "pavement quality index (PQI) average" quantitative
variable \\
\hline
$X_5$ and ln$X_5$ & "road section length" quantitative variable
and its logarithm \\
\hline
$X_{15}$ & "number of lanes on a roadway" quantitative variable \\
\hline
$X_{20}$ & "median barrier presence" indicator variable \\
\hline
$X_{23}$ & "interior shoulder presence" indicator variable \\
\hline
$X_{27}$ & "outside shoulder width" quantitative variable \\
\hline
$X_{32}$ and ln$X_{32}$ & "Average Annual Daily Traffic
(annual average)" quantitative variable and its logarithm \\
\hline
$X_{34}$ & "posted speed limit" quantitative variable \\
\hline
$X_{62}$ & "number of vertical curves per roadway section"
quantitative variable \\
\hline
$X_{64}$ & "percentage of single unit trucks (daily average)"
quantitative variable \\
\hline
$X_{66}$ & "number of changes per vertical profile along a roadway section"
quantitative variable \\
\hline
\end{tabular}



==> severity_expl-stat_table.tex <==

\begin{longtable}{|l|l|c|c|c|c|c|}
  \caption{Explanations and summary statistics for variables and parameters listed in Tables~\ref{T_interst_one-veh}--\ref{T_street_two-veh}}\\
  \hline
${\bf Variable}$ &
${\bf Description}$ &
${\bf Mean}$ &
${\bf Std}^{\,\rm a}$ &
${\bf Min}^{\,\rm a}$ &
${\bf Median}$ &
${\bf Max}^{\,\rm a}$
\\
  \hline \endfirsthead
  \caption[]{\emph{continued}}\\
  \hline
${\bf Variable}$ &
${\bf Description}$ &
${\bf Mean}$ &
${\bf Std}^{\,\rm a}$ &
${\bf Min}^{\,\rm a}$ &
${\bf Median}$ &
${\bf Max}^{\,\rm a}$
\\
  \hline \endhead
  \hline
  \multicolumn{7}{r}{\emph{continued on next page}}
  \endfoot
  \hline\endlastfoot
age0 &
Age of the driver at fault is less than $18$ years old (dummy) &
$.0846$ &
$.278$ &
$0$ &
$0$ &
$1.00$
\\
\hline
age0o &
Age of the oldest driver involved into the accident is less than $18$ years old (dummy) &
$.0103$ &
$.101$ &
$0$ &
$0$ &
$1.00$
\\
\hline
cons &
Construction at the accident location (dummy) &
$.0272$ &
$.163$ &
$0$ &
$0$ &
$1.00$
\\
\hline
curve &
Roadway is at curve (dummy) &
$.0459$ &
$.209$ &
$0$ &
$0$ &
$1.00$
\\
\hline
dark &
Dark time with no street lights (dummy) &
$.0439$ &
$.205$ &
$0$ &
$0$ &
$1.00$
\\
\hline
darklamp &
Dark and street lights on (dummy) &
$.130$ &
$.337$ &
$0$ &
$0$ &
$1.00$
\\
\hline
day &
Daylight (dummy) &
$.784$ &
$.412$ &
$0$ &
$1.00$ &
$1.00$
\\
\hline
dayt &
Day hours: 9:00 to 17:00 (dummy) &
$.577$ &
$.495$ &
$0$ &
$1.00$ &
$1.00$
\\
\hline
driv &
Roadway median is drivable (dummy) &
$.415$ &
$.493$ &
$0$ &
$0$ &
$1.00$
\\
\hline
driver &
Primary cause of the accident is driver-related (dummy) &
$.964$ &
$.185$ &
$0$ &
$1.00$ &
$1.00$
\\
\hline
dry &
Roadway surface is dry (dummy) &
$.739$ &
$.439$ &
$0$ &
$1.00$ &
$1.00$
\\
\hline
env &
Primary cause of the accident is environment-related (dummy) &
$.0255$ &
$.158$ &
$0$ &
$0$ &
$1.00$
\\
\hline
hl10 &
Help arrived in 10 minutes or less after the crash (dummy) &
$.637$ &
$.481$ &
$0$ &
$1.00$ &
$1.00$
\\
\hline
hl20 &
Help arrived in 20 minutes or less after the crash (dummy) &
$.834$ &
$.372$ &
$0$ &
$1.00$ &
$1.00$
\\
\hline
Ind &
License state of the vehicle at fault is Indiana (dummy) &
$.907$ &
$.290$ &
$0$ &
$1.00$ &
$1.00$
\\
\hline
light &
Daylight or street lights are lit up if dark (dummy) &
$.914$ &
$.281$ &
$0$ &
$1.00$ &
$1.00$
\\
\hline
maxpass &
The largest number of occupants in all vehicles involved &
$1.88$ &
$1.77$ &
$0$ &
$$ &
$70.0$
\\
\hline
mm &
Two male drivers are involved, if a 2-vehicle accident (dummy) &
$.308$ &
$.461$ &
$0$ &
$0$ &
$1.00$
\\
\hline
morn &
Morning hours: 5:00 to 9:00 (dummy) &
$.131$ &
$.337$ &
$0$ &
$0$ &
$1.00$
\\
\hline
moto &
The vehicle at fault is a motorcycle (dummy) &
$.00348$ &
$.0589$ &
$0$ &
$0$ &
$1.00$
\\
\hline
nigh &
Late night hours: 1:00 to 5:00 (dummy) &
$.0148$ &
$.121$ &
$0$ &
$0$ &
$1.00$
\\
\hline
nocons &
No construction at the accident location (dummy) &
$.973$ &
$.163$ &
$0$ &
$1.00$ &
$1.00$
\\
\hline
nojun &
No roadway junction at the accident location (dummy) &
$.448$ &
$.497$ &
$0$ &
$1.00$ &
$1.00$
\\
\hline
nonroad &
Non-roadway crash (parking lot, etc.) (dummy) &
$.00518$ &
$.0718$ &
$0$ &
$0$ &
$1.00$
\\
\hline
nosig &
No any traffic control device for the vehicle at fault (dummy) &
$.233$ &
$.423$ &
$0$ &
$0$ &
$1.00$
\\
\hline
olddrv &
The driver at fault is older than the other driver, if a 2-vehicle accident (dummy) &
$47.3$ &
$16.5$ &
$15.0$ &
$$ &
$99.0$
\\
\hline
oldvage &
Age of the oldest vehicle involved (in years) &
$10.2$ &
$5.07$ &
$-1.00$ &
$$ &
$41.0$
\\
\hline
othUS &
License state of the vehicle at fault is a U.S. state except Indiana and its neighboring
& & & & &\\
&
states (IL, KY, OH, MI) (dummy) &
$.0272$ &
$.148$ &
$0$ &
$0$ &
$1.00$
\\
\hline
precip &
Precipitation: rain/freezing rain/snow/sleet/hail (dummy) &
$.172$ &
$.377$ &
$0$ &
$0$ &
$1.00$
\\
\hline
priv &
Road traveled by the vehicle at fault is a private drive (dummy) &
$.0289$ &
$.168$ &
$0$ &
$0$ &
$1.00$
\\
\hline
r21 &
Roadway traveled by the vehicle at fault is two-lane and one-way (dummy) &
$.0347$ &
$.183$ &
$0$ &
$0$ &
$1.00$
\\
\hline
rmd2 &
Roadway traveled by the vehicle at fault is multi-lane and divided two-way (dummy) &
$.230$ &
$.421$ &
$0$ &
$0$ &
$1.00$
\\
\hline
singSUV &
One of the two vehicles involved is a pickup OR a van OR a sport utility vehicle,
& & & & &\\
&
if a 2-vehicle accident (dummy) &
$.446$ &
$.497$ &
$0$ &
$0$ &
$1.00$
\\
\hline
singTR &
One of the two vehicles is a truck OR a tractor, if a 2-vehicle accident (dummy) &
$.0688$ &
$.253$ &
$0$ &
$0$ &
$1.00$
\\
\hline
slush &
Roadway surface is covered by snow/slush (dummy) &
$.0400$ &
$.196$ &
$0$ &
$0$ &
$1.00$
\\
\hline
snow &
Snowing weather (dummy) &
$.0414$ &
$.199$ &
$0$ &
$0$ &
$1.00$
\\
\hline
str &
Roadway is straight (dummy) &
$.949$ &
$.220$ &
$0$ &
$1.00$ &
$1.00$
\\
\hline
sum &
Summer season (dummy) &
$.243$ &
$.429$ &
$0$ &
$0$ &
$1.00$
\\
\hline
sund &
Sunday (dummy) &
$.0784$ &
$.269$ &
$0$ &
$0$ &
$1.00$
\\
\hline
thday &
Thursday (dummy) &
$.157$ &
$.364$ &
$0$ &
$0$ &
$1.00$
\\
\hline
vage &
Age of the vehicle at fault (in years) &
$7.91$ &
$5.31$ &
$-1.00$ &
$$ &
$41.0$
\\
\hline
voldg &
The vehicle at fault is more than 7 years old (dummy) &
$.489$ &
$.500$ &
$0$ &
$0$ &
$1.00$
\\
\hline
voldo &
Age of the oldest vehicle involved is more than 7 years (dummy) &
$.688$ &
$.463$ &
$0$ &
$1.00$ &
$1.00$
\\
\hline
wall &
Road median is a wall (dummy) &
$.0528$ &
$.224$ &
$0$ &
$0$ &
$1.00$
\\
\hline
way4 &
Accident location is at a 4-way intersection (dummy) &
$.371$ &
$.483$ &
$0$ &
$0$ &
$1.00$
\\
\hline
wday &
Weekday (Monday through Friday) (dummy) &
$.800$ &
$.400$ &
$0$ &
$1.00$ &
$1.00$
\\
\hline
wint &
Winter season (dummy) &
$.250$ &
$.433$ &
$0$ &
$0$ &
$1.00$
\\
\hline
$X_{12}$ &
Roadway type (dummy: 1 if urban, 0 if rural) &
$.829$ &
$.377$ &
$0$ &
$1.00$ &
$1.00$
\\
\hline
$X_{27}$ &
Number of occupants in the vehicle at fault &
$1.45$ &
$1.18$ &
$0$ &
$$ &
$70.0$
\\
\hline
$X_{29}$ &
Speed limit (used if known and the same for all vehicles involved) &
$36.7$ &
$9.86$ &
$5.00$ &
$$ &
$75.0$
\\
\hline
$X_{33}$ &
At least one of the vehicles involved was on fire (dummy) &
$.00505$ &
$.0709$ &
$0$ &
$0$ &
$1.00$
\\
\hline
$X_{34}$ &
Age of the driver at fault (in years) &
$37.0$ &
$9.86$ &
$3.00$ &
$$ &
$99.0$
\\
\hline
$X_{35}$ &
Gender of the driver at fault (dummy: 1 if female, 0 if male) &
$.449$ &
$.497$ &
$0$ &
$0$ &
$1.00$
\\
\hline
\hline
$\langle P_{t,n}^{(i)}\rangle_X$ &
Probability of $i^{\rm th}$ severity outcome averaged over all values
of explanatory variables ${\bf X}_{t,n}$ &
-- &
-- &
-- &
-- &
--
\\
\hline
$p_{0\rightarrow1}$ &
Markov transition probability of jump $0\to1$, as time $t$ increases to $t+1$ &
-- &
-- &
-- &
-- &
--
\\
\hline
$p_{1\rightarrow0}$ &
Markov transition probability of jump $1\to0$, as time $t$ increases to $t+1$ &
-- &
-- &
-- &
-- &
--
\\
\hline
${\bar p}_0$ and ${\bar p}_1$ &
Unconditional probabilities of states 0 and 1 &
-- &
-- &
-- &
-- &
--
\\
\hline
$\#$ free par. &
Total number of free model parameters ($\beta$-s) &
-- &
-- &
-- &
-- &
--
\\
\hline
averaged $LL\!$ &
Posterior average of the log-likelihood (LL) &
-- &
-- &
-- &
-- &
--
\\
\hline
$\max(LL)$ &
True maximum value of log-likelihood (LL) for MLE; maximum observed value of LL & & & & & \\
& for Bayesian-MCMC &
-- &
-- &
-- &
-- &
--
\\
\hline
marginal $LL\!$ &
Logarithm of marginal likelihood of data ($\ln[f({\bf Y}|{\cal M})]$) &
-- &
-- &
-- &
-- &
--
\\
\hline
max(PSRF) &
Maximum of the potential scale reduction factors$^{\,\rm b}$ &
-- &
-- &
-- &
-- &
--
\\
\hline
MPSRF &
Multivariate potential scale reduction factor (MPSRF)$^{\,\rm b}$ &
-- &
-- &
-- &
-- &
--
\\
%\hline
%accept. rate &
%Average candidate acceptance rate in Metropolis-Hasting sampling &
%-- &
%-- &
%-- &
%-- &
%--
%\\
\hline
$\#$ observ. &
number of observations of accident severity outcomes available in the data sample &
-- &
-- &
-- &
-- &
--
\\
\hline
\multicolumn{7}{l}{$^{\rm a}$ Standard deviation, minimum and maximum of a variable.}\\
\multicolumn{7}{l}{$^{\rm b}$ PSRF/MPSRF are calculated separately/jointly for all continuous model parameters. PSRF and MPSRF are close to 1 for converged MCMC chains.}
\end{longtable}












==> severity_expl_table_a.tex <==

\begin{tabular}{|l|l|}
\hline
\bf Variable & \hspace{4cm}{\bf Description}\\
\hline
$\langle P_{t,n}^{(i)}\rangle_X$ & probability of $i^{\rm th}$ severity
outcome averaged over all values of explanatory variables ${\bf X}_{t,n}$\\
\hline
$p_{0\rightarrow1}$ & Markov transition probability of jump from
state 0 to state 1 as time $t$ increases to $t+1$\\
\hline
$p_{1\rightarrow0}$ & Markov transition probability of jump from
state 1 to state 0 as time $t$ increases to $t+1$\\
\hline
${\bar p}_0$ and ${\bar p}_1$ & unconditional probabilities of
states 0 and 1\\
\hline
$\#$ free par. & total number of free model coefficients ($\beta$-s)\\
\hline
averaged $LL\!$ & posterior average of the log-likelihood (LL)\\
\hline
$\max(LL)$ & for MLE it is the maximal value of $LL$ at convergence;
for Bayesian-MCMC estimation \\
& it is the maximal observed value of LL during the MCMC simulations\\
\hline
marginal $LL\!$ & logarithm of marginal likelihood of data,
$\ln[f({\bf Y}|{\cal M})]$, given model ${\cal M}$\\
\hline
max(PSRF) & maximum of the potential scale reduction factors (PSRF)
calculated separately for all \\
& continuous model parameters, PSRF is close to 1 for converged
MCMC chains\\
\hline
MPSRF & multivariate PSRF calculated jointly for all parameters,
close to 1 for converged MCMC\\
\hline
accept. rate & average rate of acceptance of candidate values
during Metropolis-Hasting MCMC draws\\
\hline
$\#$ observ. & number of observations of accident severity
outcomes available in the data sample\\
\hline
\hline
age0 & "age of the driver at fault is $<18$ years" indicator variable
(dummy)\\
\hline
age0o & "age of the oldest driver involved into the accident is $<18$ years"
indicator variable\\
\hline
cons & "construction at the accident location" indicator variable\\
\hline
curve & "road is at curve" indicator variable\\
\hline
dark & "dark time with no street lights" indicator variable\\
\hline
darklamp & "dark AND street lights on" indicator variable\\
\hline
day & "daylight" indicator variable\\
\hline
dayt & "day hours: 9:00 to 17:00" indicator variable\\
\hline
driv & "road median is drivable" indicator variable\\
\hline
driver & "primary cause of the accident is driver-related" indicator
variable\\
\hline
dry & "roadway surface is dry" indicator variable\\
\hline
env & "primary cause of the accident is environment-related" indicator
variable\\
\hline
fog & "fog OR smoke OR smog" indicator variable\\
\hline
hl10 & "help arrived in 10 minutes or less after the crash" indicator
variable\\
\hline
hl20 & "help arrived in 20 minutes or less after the crash" indicator
variable\\
\hline
Ind & "license state of the vehicle at fault is Indiana" indicator
variable\\
\hline
intercept & "constant term (intercept)" quantitative variable\\
\hline
jobend & "after work hours: from 16:00 to 19:00" indicator variable\\
\hline
light & "daylight OR street lights are lit up if dark"
indicator variable\\
\hline
maxpass & "the largest number of occupants in all vehicles involved"
quantitative variable\\
\hline
mm & "two male drivers are involved" indicator
variable (used only if a 2-vehicle accident)\\
\hline
morn & "morning hours: 5:00 to 9:00" indicator variable\\
\hline
moto & "the vehicle at fault is a motorcycle" indicator variable\\
\hline
\end{tabular}






==> severity_expl_table_b.tex <==

\begin{tabular}{|l|l|}
\hline
\bf Variable & \hspace{4cm}{\bf Description}\\
\hline
nigh & "late night hours: 1:00 to 5:00" indicator variable\\
\hline
nocons & "no construction at the accident location" indicator variable\\
\hline
nojun & "no road junction at the accident location" indicator variable\\
\hline
nonroad & "non-roadway crash (parking lot, etc.)" indicator variable\\
\hline
nosig & "no any traffic control device for the vehicle at fault"
indicator variable\\
\hline
olddrv & "the driver at fault is older than the other driver"
indicator var. (if a 2-vehicle accident)\\
\hline
oldvage & "age (in years) of the oldest vehicle involved" indicator variable\\
\hline
othUS & "license state of the vehicle at fault is a U.S. state except
Indiana and its neighboring\\
& states (IL, KY, OH, MI)" indicator variable\\
\hline
precip & "precipitation: rain OR snow OR sleet OR hail OR freezing rain"
indicator variable\\
\hline
priv & "road traveled by the vehicle at fault is a private drive"
indicator variable\\
\hline
r21 & "road traveled by the vehicle at fault is two-lane AND one-way"
indicator variable\\
\hline
rmd2 & "road traveled by the vehicle at fault is multi-lane AND divided
two-way" indicator var.\\
\hline
singSUV & "one of the two vehicles involved is a pickup OR a van OR
a sport utility vehicle"\\
& indicator variable (used only if a 2-vehicle accident)\\
\hline
singTR & "one of the two vehicles is a truck OR a tractor"
indicator var. (if a 2-vehicle accident)\\
\hline
slush & "roadway surface is covered by snow/slush" indicator variable\\
\hline
snow & "snowing weather" indicator variable\\
\hline
str & "road is straight" indicator variable\\
\hline
sum & "summer season" indicator variable\\
\hline
sund & "Sunday" indicator variable\\
\hline
thday & "Thursday" indicator variable\\
\hline
vage & "age (in years) of the vehicle at fault" quantitative variable\\
\hline
veh & "primary cause of accident is vehicle-related" indicator variable\\
\hline
voldg & "the vehicle at fault is more than 7 years old" indicator variable\\
\hline
voldo & "age of the oldest vehicle involved is more than 7 years" indicator
variable\\
\hline
wall & "road median is a wall" indicator variable\\
\hline
way4 & "accident location is at a 4-way intersection" indicator variable\\
\hline
wday & "weekday (Monday through Friday)" indicator variable\\
\hline
wint & "winter season" indicator variable\\
\hline
$X_{12}$ & "road type" indicator variable (1 if urban, 0 if rural)\\
\hline
$X_{27}$ & "number of occupants in the vehicle at fault"
quantitative variable\\
\hline
$X_{29}$ & "speed limit" quantitative var. (used if known and
the same for all vehicles involved)\\
\hline
$X_{33}$ & "at least one of the vehicles involved was on fire"
indicator variable\\	
\hline
$X_{34}$ & "age (in years) of the driver at fault" quantitative
variable\\
\hline
$X_{35}$ & "gender of the driver at fault" indicator
variable (1 if female, 0 if male)\\
\hline
\end{tabular}



==> severity_statistics_table_a.tex <==

\tabcolsep=0.5em

\begin{tabular}{|l|c|c|c|c|c|}
\hline
${\bf Variable}$ &
${\bf Mean}$ &
${\bf Std}^{\,\rm a}$ &
${\bf Min}^{\,\rm a}$ &
${\bf Median}$ &
${\bf Max}^{\,\rm a}$
\\
\hline
Summer season (dummy) &
$.243$ &
$.429$ &
$0$ &
$0$ &
$1.00$
\\
\hline
Thursday (dummy) &
$.157$ &
$.364$ &
$0$ &
$0$ &
$1.00$
\\
\hline
Construction at the accident location (dummy) &
$.0272$ &
$.163$ &
$0$ &
$0$ &
$1.00$
\\
\hline
Daylight or street lights are lit up if dark (dummy) &
$.914$ &
$.281$ &
$0$ &
$1.00$ &
$1.00$
\\
\hline
Precipitation: rain/freezing rain/snow/sleet/hail (dummy) &
$.172$ &
$.377$ &
$0$ &
$0$ &
$1.00$
\\
\hline
Roadway surface is covered by snow/slush (dummy) &
$.0400$ &
$.196$ &
$0$ &
$0$ &
$1.00$
\\
\hline
Roadway median is drivable (dummy) &
$.415$ &
$.493$ &
$0$ &
$0$ &
$1.00$
\\
\hline
Roadway is at curve (dummy) &
$.0459$ &
$.209$ &
$0$ &
$0$ &
$1.00$
\\
\hline
Primary cause of the accident is driver-related (dummy) &
$.964$ &
$.185$ &
$0$ &
$1.00$ &
$1.00$
\\
\hline
Help arrived in 20 minutes or less after the crash (dummy) &
$.834$ &
$.372$ &
$0$ &
$1.00$ &
$1.00$
\\
\hline
The vehicle at fault is a motorcycle (dummy) &
$.00348$ &
$.0589$ &
$0$ &
$0$ &
$1.00$
\\
\hline
Age of the vehicle at fault (in years) &
$7.91$ &
$5.31$ &
$-1.00$ &
$$ &
$41.0$
\\
\hline
Number of occupants in the vehicle at fault &
$1.45$ &
$1.18$ &
$0$ &
$$ &
$70.0$
\\
\hline
Roadway traveled by the vehicle at fault is multi-lane and
& & & & &\\
divided two-way (dummy) &
$.230$ &
$.421$ &
$0$ &
$0$ &
$1.00$
\\
\hline
At least one of the vehicles involved was on fire (dummy) &
$.00505$ &
$.0709$ &
$0$ &
$0$ &
$1.00$
\\
\hline
Gender of the driver at fault (dummy: 1 if female, 0 if male) &
$.449$ &
$.497$ &
$0$ &
$0$ &
$1.00$
\\
\hline
Snowing weather (dummy) &
$.0414$ &
$.199$ &
$0$ &
$0$ &
$1.00$
\\
\hline
No roadway junction at the accident location (dummy) &
$.448$ &
$.497$ &
$0$ &
$1.00$ &
$1.00$
\\
\hline
Roadway is straight (dummy) &
$.949$ &
$.220$ &
$0$ &
$1.00$ &
$1.00$
\\
\hline
Primary cause of the accident is environment-related (dummy) &
$.0255$ &
$.158$ &
$0$ &
$0$ &
$1.00$
\\
\hline
Help arrived in 10 minutes or less after the crash (dummy) &
$.637$ &
$.481$ &
$0$ &
$1.00$ &
$1.00$
\\
\hline
Speed limit (used if known and the same for all vehicles involved) &
$36.7$ &
$9.86$ &
$5.00$ &
$$ &
$75.0$
\\
\hline
Roadway traveled by the vehicle at fault is two-lane and
& & & & &\\
one-way (dummy) &
$.0347$ &
$.183$ &
$0$ &
$0$ &
$1.00$
\\
\hline
Age of the driver at fault (in years) &
$37.0$ &
$9.86$ &
$3.00$ &
$$ &
$99.0$
\\
\hline
Weekday (Monday through Friday) (dummy) &
$.800$ &
$.400$ &
$0$ &
$1.00$ &
$1.00$
\\
\hline
Roadway type (dummy: 1 if urban, 0 if rural) &
$.829$ &
$.377$ &
$0$ &
$1.00$ &
$1.00$
\\
\hline
License state of the vehicle at fault is a U.S. state except Indiana
& & & & &\\
and its neighboring states (IL, KY, OH, MI) (dummy) &
$.0272$ &
$.148$ &
$0$ &
$0$ &
$1.00$
\\
%=== Additional variables to the paper with severity models ===
\hline
Late night hours: 1:00 to 5:00 (dummy) &
$.0148$ &
$.121$ &
$0$ &
$0$ &
$1.00$
\\
\hline
Dark time with no street lights (dummy) &
$.0439$ &
$.205$ &
$0$ &
$0$ &
$1.00$
\\
\hline
Age of the oldest vehicle involved (in years) &
$10.2$ &
$5.07$ &
$-1.00$ &
$$ &
$41.0$
\\
\hline
The largest number of occupants in all vehicles involved &
$1.88$ &
$1.77$ &
$0$ &
$$ &
$70.0$
\\
\hline
Two male drivers are involved, if a 2-vehicle accident (dummy) &
$.308$ &
$.461$ &
$0$ &
$0$ &
$1.00$
\\
\hline
\multicolumn{6}{l}{$^{\rm a}$ Standard deviation, minimum and maximum of a variable.}\\
\end{tabular}









==> severity_statistics_table_b.tex <==

\tabcolsep=0.5em

\begin{tabular}{|l|c|c|c|c|c|}
\hline
${\bf Variable}$ &
${\bf Mean}$ &
${\bf Std}^{\,\rm a}$ &
${\bf Min}^{\,\rm a}$ &
${\bf Median}$ &
${\bf Max}^{\,\rm a}$
\\
\hline
Winter season (dummy) &
$.250$ &
$.433$ &
$0$ &
$0$ &
$1.00$
\\
\hline
Day hours: 9:00 to 17:00 (dummy) &
$.577$ &
$.495$ &
$0$ &
$1.00$ &
$1.00$
\\
\hline
Road traveled by the vehicle at fault is a private drive (dummy) &
$.0289$ &
$.168$ &
$0$ &
$0$ &
$1.00$
\\
\hline
One of the two vehicles is a truck OR a tractor, if a 2-vehicle
& & & & &\\
accident (dummy) &
$.0688$ &
$.253$ &
$0$ &
$0$ &
$1.00$
\\
\hline
The driver at fault is older than the other driver, if a 2-vehicle
& & & & &\\
accident (dummy) &
$47.3$ &
$16.5$ &
$15.0$ &
$$ &
$99.0$
\\
\hline
Road median is a wall (dummy) &
$.0528$ &
$.224$ &
$0$ &
$0$ &
$1.00$
\\
\hline
Age of the oldest vehicle involved is more than 7 years (dummy) &
$.688$ &
$.463$ &
$0$ &
$1.00$ &
$1.00$
\\
\hline
No construction at the accident location (dummy) &
$.973$ &
$.163$ &
$0$ &
$1.00$ &
$1.00$
\\
\hline
Daylight (dummy) &
$.784$ &
$.412$ &
$0$ &
$1.00$ &
$1.00$
\\
\hline
Sunday (dummy) &
$.0784$ &
$.269$ &
$0$ &
$0$ &
$1.00$
\\
\hline
Morning hours: 5:00 to 9:00 (dummy) &
$.131$ &
$.337$ &
$0$ &
$0$ &
$1.00$
\\
\hline
Dark and street lights on (dummy) &
$.130$ &
$.337$ &
$0$ &
$0$ &
$1.00$
\\
\hline
Accident location is at a 4-way intersection (dummy) &
$.371$ &
$.483$ &
$0$ &
$0$ &
$1.00$
\\
\hline
One of the two vehicles involved is a pickup OR a van OR a sport
& & & & &\\
utility vehicle, if a 2-vehicle accident (dummy) &
$.446$ &
$.497$ &
$0$ &
$0$ &
$1.00$
\\
\hline
Age of the driver at fault is less than $18$ years old (dummy) &
$.0846$ &
$.278$ &
$0$ &
$0$ &
$1.00$
\\
\hline
Age of the oldest driver involved into the accident is less than $18$
& & & & &\\
years old (dummy) &
$.0103$ &
$.101$ &
$0$ &
$0$ &
$1.00$
\\
\hline
Roadway surface is dry (dummy) &
$.739$ &
$.439$ &
$0$ &
$1.00$ &
$1.00$
\\
\hline
License state of the vehicle at fault is Indiana (dummy) &
$.907$ &
$.290$ &
$0$ &
$1.00$ &
$1.00$
\\
\hline
Non-roadway crash (parking lot, etc.) (dummy) &
$.00518$ &
$.0718$ &
$0$ &
$0$ &
$1.00$
\\
\hline
The vehicle at fault is more than 7 years old (dummy) &
$.489$ &
$.500$ &
$0$ &
$0$ &
$1.00$
\\
\hline
No any traffic control device for the vehicle at fault (dummy) &
$.233$ &
$.423$ &
$0$ &
$0$ &
$1.00$
\\
\hline
\multicolumn{6}{l}{$^{\rm a}$ Standard deviation, minimum and maximum of a variable.}\\
\end{tabular}








